SIEVE: Effective Filtered Vector Search with Collection of Indexes

Many real-world tasks such as recommending videos with the kids tag can be reduced to finding most similar vectors associated with hard predicates. This task, filtered vector search, is challenging as prior state-of-the-art graph-based (unfiltered) similarity search techniques quickly degenerate when hard constraints are considered. That is, effective graph-based filtered similarity search relies on sufficient connectivity for reaching the most similar items within just a few hops. To consider predicates, recent works propose modifying graph traversal to visit only the items that may satisfy predicates. However, they fail to offer the just-a-few-hops property for a wide range of predicates: they must restrict predicates significantly or lose efficiency if only a small fraction of items satisfy predicates. We propose an opposite approach: instead of constraining traversal, we build many indexes each serving different predicate forms. For effective construction, we devise a three-dimensional analytical model capturing relationships among index size, search time, and recall, with which we follow a workload-aware approach to pack as many useful indexes as possible into a collection. At query time, the analytical model is employed yet again to discern the one that offers the fastest search at a given recall. We show superior performance and support on datasets with varying selectivities and forms: our approach achieves up to 8.06x speedup while having as low as 1% build time versus other indexes, with less than 2.15x memory of a standard HNSW graph and modest knowledge of past workloads.

==> sections/algorithms/construction.tex <==
\setlength{\textfloatsepsave}{\textfloatsep} \setlength{\textfloatsep}{1pt}
\begin{algorithm}[t]
% \small
\caption{\system\_Construct\_Index \label{alg:construction}}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Dataset $(\mathcal{D}, \mathcal{A})$, Historical Filters $(\mathcal{H})$, index memory budget $B$
}
\Output{Index collection $\mathcal{I}$ with total size bounded by $M$}
$\mathcal{I} = \mathcal{F}$\\
\While{$sum_{I_h\in \mathcal{I}}S(I_h) > M$}{
    $I_{worst} = argmin{I_h\in \mathcal{I}}\frac{C(\mathcal{I}, \mathcal{H})-C(\mathcal{I}-\{I_h\}, \mathcal{H})}{card(h)}$\\
    $\mathcal{I} = \mathcal{I} - \{I_{worst}\}$\\
}

\textbf{Return} $\mathcal{I}$.\\
\end{algorithm}

==> sections/algorithms/serving.tex <==
\setlength{\textfloatsepsave}{\textfloatsep} \setlength{\textfloatsep}{1pt}
\begin{algorithm}[t]
% \small
\caption{\system\_Serve\_Knn\_Query \label{alg:serving}}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{query vector $q$, query filter $f$, search parameters $(k, ef\_search)$, index collection $\mathcal{I}$, dataset $(\mathcal{D}, \mathcal{A})$
}
\Output{$k$ closest vectors in $(\mathcal{D}, \mathcal{A})$ to $q$ satisfying filter $f$}
$I_{h}=argmin_{I_h\in \{I_h|I_h \in \mathcal{I}, h\,\text{subsumes}\,f\}}card(h)$  // BFS over $\mathcal{I}$\\
$cost_{index} = \frac{ef\_search\times c(I_h, f)}{ef\_construction}$\\
$cost_{bruteforce} = c_{bf}(\mathcal{D}, \mathcal{A}, f)$\\
\If{$cost_{index} < cost_{bruteforce}$}{
  \textbf{Return} $SearchKNN(I_h, q, f, k, ef\_search)$.\\
}
\textbf{Return} $SearchBruteforce(\mathcal{D}, \mathcal{A}, q, f, k)$.
\end{algorithm}

==> sections/tables/experiment_distcomps.tex <==
\begin{table}[t]

\caption{\system's average number of distance computations per query to achieve 0.95 recall.}
\vspace{-3mm}
\footnotesize
\addtolength{\tabcolsep}{-3pt} 
\midsepremove
\begin{tabular}{|l|c|c|c|c|c|}
\toprule
 & \multicolumn{5}{c|}{Dataset}\\
  \midrule
 Method & \yfcc & \paper & \uqv & \sift & \msong \\
  \midrule
\cellcolor{gray!25} \oracle & \cellcolor{gray!25} 534.7 & \cellcolor{gray!25} 423.1 & \cellcolor{gray!25} 338.9 & \cellcolor{gray!25} 1128.7 & \cellcolor{gray!25} 1114.7\\
 \midrule
\smarthnsw & 10726.4 & 10009.7 & 4170.8 & 5685.4 & 3015.2\\
 \midrule
 % \hnswbase & 1660935 & 28805.6 & 14030.2 & 5691.6 & 2416.7\\
 % \midrule
 \caps & N/A & N/A & N/A & 12000 & 18000 \\
 \midrule
 \acornone & N/A & \textbf{1606.0} & 1289.0 & 2886.2 & 6053.59 \\
 \midrule
\acorngamma & N/A & 1634.6 & 1019.1 & 1478.1 & 1776.3 \\
 \midrule
\parlayivf & \textbf{1775.9} & N/A & N/A & \textbf{1156.9} & N/A \\
 \midrule
\system & 2368.0 & 4273.9 & 1637.6 & 4181.8 & 2675.9\\
%3039.3 at 0.93 for acornone on yfcc
\bottomrule
\end{tabular}
\midsepdefault
\addtolength{\tabcolsep}{3pt}
\vspace{-2mm}
\label{tbl:experiment_fast_capture}
\end{table}
% \smarthnsw & 8166.2 & 9858.5 & 3984.5 & 3964.6 & 1874.5\\
%  \midrule

==> sections/tables/experiment_update_workload.tex <==
\begin{table}[t]

\caption{\systemnosf's update time from an initial index collection fit with 25\% of query workload to an updated index collection fit with 100\% of query workload.}
% \silu{do we need to update the percentile here? If not, we can call out this is the index size without vector data.}
% \billy{The percentiles have already been updated.}
\vspace{-3mm}
\footnotesize
\addtolength{\tabcolsep}{-2pt} 
\midsepremove

\begin{tabular}{ l r  r r r}
\toprule
\multirow{2}{*}{Dataset} & Update time (s) & \multirow{2}{*}{Subindex \# change} & New subindexes size (GB) \\
&  (\% of init. time) &  & (\% of original size) \\
  \midrule
\yfcc  & 12.738 (9.62\%) & 658$\rightarrow$604 (-172, +118) & 1.388 (8.31\%) \\
\paper  & 12.280 (19.6\%) & 186$\rightarrow$201 (-55, +70) & 0.723 (13.7\%) \\
\uqv  & 3.985 (23.5\%) & 168$\rightarrow$176 (-55, +63) & 0.444 (14.1\%) \\
\sift  & 2.238 (7.91\%) & 23$\rightarrow$23 (-4, +4) & 0.225 (6.76\%) \\
\msong  & 0 (0\%) & 8$\rightarrow$8 (0, 0) & 0 (0\%) \\

\bottomrule
\end{tabular}
\midsepdefault
\addtolength{\tabcolsep}{2pt}
\vspace{-4mm}
\label{tbl:experiment_update_times}
\end{table}
% \smarthnsw & 8166.2 & 9858.5 & 3984.5 & 3964.6 & 1874.5\\
%  \midrule

